Optimal transport with constraints: from mirror descent to classical mechanics

Finding optimal trajectories for multiple traffic demands in a congested network is a challenging task. Optimal transport theory is a principled approach that has been used successfully to study various transportation problems. Its usage is limited by the lack of principled and flexible ways to incorporate realistic constraints. We propose a principled physics-based approach to impose constraints flexibly in such optimal transport problems. Constraints are included in mirror descent dynamics using the principle of D'Alembert-Lagrange from classical mechanics. This leads to a sparse, local and linear approximation of the feasible set leading in many cases to closed-form updates.

==> related_work.tex <==
\section{Related work}
%should be no more than 1-2 PRL pages (<2000
%words)
Optimizing transport on networks is a multifaceted problem. Accordingly, it has been addressed from different angles over the last decades. \\
In operation research there is a large literature about network flows \cite{ahuja1988network}, 
in particular minimum-cost optimization is relevant to our goal. It aims at finding a flow that minimizes a given total cost function, given a set of costs assigned to individual network edges, in addition to satisfing a set of constraints. Shortest-path optimization is a relevant example. Typically, these settings consider discrete flows and can be solved using classical techniques from linear programming, e.g. cycle canceling,  network simplex or Ford–Fulkerson algorithms.
In our work we consider instead the continuous case, where flows (and conductivities) are real-valued quantities. In this context, optimal transport \cite{santambrogio2015optimal} classifies problems structured similarly to
minimum-cost flow as the 1-Wasserstein distance or Beckmann problem \cite{beckmann1952continuous}. Our approach falls into this category, and specifically follows the perspective of a dynamical formulation where the solution of the optimization problem is obtained by solving a dynamical system of equations \cite{peyre2019computational}. The main advantages of this approach, over standard optimization approaches, are: numerical efficiency, as the computational cost scales conveniently with the size of the system; it allows for natural physical interpretations using analogies with fluid dynamics in electrical or hydraulic networks; it admits theoretical derivations that formally characterize the validity of solutions.\\
Importantly, our approach takes into account traffic congestions flexibly, while many existing routing algorithms are mostly
focusing on minimizing path lengths and are insensitive to traffic congestion. In our case, one parameter allows to tune between opposite traffic regimes where one
can consolidate or discourage traffic congestion. 
Path optimality and congestion control have been studied within the physics community in other contexts, e.g. in investigating spanning \cite{noh2002stability,dobrin2001minimum} or Steiner
trees \cite{bayati2008statistical}. All these approaches are typically valid for discrete flows and are usually computationally more intensive than optimal transport-based problems in the continuous setting. 
Other approaches consider the cavity method \cite{yeung2012competition,yeung2013physics}. These usually require to specify ad-hoc algorithmic updates based on what specific constraints are considered, with computational complexity also depending on these choices. Instead, here we provide a general mechanism that can be solved for arbitrary constraints, provided one can compute their gradients.\\
Navigation in complex systems is a wide line of literature that focuses more on investigating the properties of flows, rather than their optimization as we do in this paper. For instance, jamming in complex networks \cite{nagatani2002physics,kerner1999physics,li2015percolation,lacasa2009jamming} focuses on investigating phase transitions between free flow to congestion; random walks or spatial interaction models \cite{barbosa2018human,zipf1946p} focus more on predicting flows based on expected behavior of passengers, or on attributes of the origin and destination locations; searchability and navigability investigate the interplay between path trajectories taken by passengers and the topological properties of the underlying network infrastructure \cite{rosvall2005searchability,estrada2023network}. These models often assume that passengers follow their shortest paths, which are selected as the flows used to study all these related questions. 
Our work can complement these research directions by providing a principled and efficient way to select flows that in many contexts could be more appropriate than shortest paths.

From a variational optimization perspective, our approach is related to successive linear and sequential quadratic programming \cite{nocedal2006,bertsekas1999,luenberger2016}. The underlying idea of these methods is to linearize the objective function and the constraints about the current iterate and to solve a local linear and/or quadratic programs. Our work improves upon these ideas and tailors these to optimal transport problems in the following way: i) we linearize a subset of constraints at every iteration, which means that the subproblem \Cref{eqn:updated_dyn} typically includes very few constraints and can be solved efficiently; ii) we introduce a non-Euclidean inner product that is adapted to optimal transport problems and is used to show that $\mathfrak{L}_{\beta_{}}$ is a Lyapunov function; iii) we provide closed-form updates in various problem instances that are practically relevant. 

